Video Decoding Energy Estimation Using Processor Events

In this paper, we show that processor events like instruction counts or cache misses can be used to accurately estimate the processing energy of software video decoders. Therefore, we perform energy measurements on an ARM-based evaluation platform and count processor level events using a dedicated profiling software. Measurements are performed for various codecs and decoder implementations to prove the general viability of our observations. Using the estimation method proposed in this paper, the true decoding energy for various recent video coding standards including HEVC and VP9 can be estimated with a mean estimation error that is smaller than 6%.

==> gfx/CacheMissWrite_SizeOfSequence_justLL_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA datassssssssssssssssss2}%
\psfrag{011}[cl][cl]{\matlabtextA LL cache miss write}%
\psfrag{012}[bc][bc]{\matlabtextA asd}%
\psfrag{013}[tc][tc]{\matlabtextA asd}%
%
%% </text>
%
%% <xscale>
%
\psfrag{000}[tc][tc]{\matlabtextA $\times10^{6}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextA $0$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $4$}%
\psfrag{004}[ct][ct]{\matlabtextA $6$}%
\psfrag{005}[ct][ct]{\matlabtextA $8$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $30$}%
%
%% </ytick>

==> gfx/CacheMissWrite_SizeOfSequence_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{013}[cl][cl]{\matlabtextA data3}%
\psfrag{014}[cl][cl]{\matlabtextA L1 csssssssache miss write}%
\psfrag{015}[cl][cl]{\matlabtextA LL cache miss write}%
\psfrag{016}[bc][bc]{\matlabtextA Energy}%
\psfrag{017}[tc][tc]{\matlabtextA DCacheWriteMiss}%
%
%% </text>
%
%% <xscale>
%
\psfrag{000}[tc][tc]{\matlabtextA $\times10^{7}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextA $0$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextA $1$}%
\psfrag{004}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextA $2$}%
\psfrag{006}[ct][ct]{\matlabtextA $2.5$}%
\psfrag{007}[ct][ct]{\matlabtextA $3$}%
\psfrag{008}[ct][ct]{\matlabtextA $3.5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{009}[rc][rc]{\matlabtextA $0$}%
\psfrag{010}[rc][rc]{\matlabtextA $10$}%
\psfrag{011}[rc][rc]{\matlabtextA $20$}%
\psfrag{012}[rc][rc]{\matlabtextA $30$}%
%
%% </ytick>

==> gfx/DataFetchOverEnergy_variousCodecs_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA VP9 - FFmpeg}%
\psfrag{011}[cl][cl]{\matlabtextA H.264 - FFmpeg}%
\psfrag{012}[cl][cl]{\matlabtextA HEVC - FFmpeg}%
\psfrag{013}[bc][bc]{\matlabtextA En}%
\psfrag{014}[tc][tc]{\matlabtextA Instr}%
%
%% </text>
%
%% <xscale>
%
\psfrag{000}[tc][tc]{\matlabtextA $\times10^{10}$}%
%
%% </xscale>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{001}[ct][ct]{\matlabtextA $0$}%
\psfrag{002}[ct][ct]{\matlabtextA $0.5$}%
\psfrag{003}[ct][ct]{\matlabtextA $1$}%
\psfrag{004}[ct][ct]{\matlabtextA $1.5$}%
\psfrag{005}[ct][ct]{\matlabtextA $2$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $30$}%
%
%% </ytick>

==> gfx/correlations_HEVC_matlabfrag.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{14}{14}\selectfont\strut}%
\psfrag{010}[cl][cl]{\matlabtextA Instr LL *10^6}%
\psfrag{011}[cl][cl]{\matlabtextA Intrs *10^{10}}%
\psfrag{012}[bc][bc]{\matlabtextA Ene}%
\psfrag{013}[tc][tc]{\matlabtextA Instr}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $1$}%
\psfrag{002}[ct][ct]{\matlabtextA $2$}%
\psfrag{003}[ct][ct]{\matlabtextA $3$}%
\psfrag{004}[ct][ct]{\matlabtextA $4$}%
\psfrag{005}[ct][ct]{\matlabtextA $5$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextA $0$}%
\psfrag{007}[rc][rc]{\matlabtextA $10$}%
\psfrag{008}[rc][rc]{\matlabtextA $20$}%
\psfrag{009}[rc][rc]{\matlabtextA $30$}%
%
%% </ytick>
